The BABAR Detector

BABAR, the detector for the SLAC PEP-II asymmetric e+e- B Factory operating at the upsilon 4S resonance, was designed to allow comprehensive studies of CP-violation in B-meson decays. Charged particle tracks are measured in a multi-layer silicon vertex tracker surrounded by a cylindrical wire drift chamber. Electromagentic showers from electrons and photons are detected in an array of CsI crystals located just inside the solenoidal coil of a superconducting magnet. Muons and neutral hadrons are identified by arrays of resistive plate chambers inserted into gaps in the steel flux return of the magnet. Charged hadrons are identified by dE/dx measurements in the tracking detectors and in a ring-imaging Cherenkov detector surrounding the drift chamber. The trigger, data acquisition and data-monitoring systems, VME- and network-based, are controlled by custom-designed online software. Details of the layout and performance of the detector components and their associated electronics and software are presented.

==> NIMsym2.tex <==
% NIMsym.tex - definitions for symbols and macros that are needed by
%              the BABAR NIM paper and are not already in either LaTeX
%              or in babarsym.tex.  Note that this file should be included
%              BEFORE babarsym.tex so that if a particular symbol/macro
%              appears in babarsym.tex, that definition will prevail.
%
%  Much of this content came from the TDR's ``symbols.tex'' file
%
%
%  T.Glanzman, 16 October 2000
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% comment is used to comment out parts of the text:
\newcommand{\comment}[1]{}

%% Define section name and section (sub)directory for each Section
% Define directory for includes; renewcommand before each chapter
\newcommand{\sectiondir}{}
% Define directory for includes; renewcommand before each chapter
\newcommand{\secname}{}

%% General english terms, and common things for formulas.
\def\etal{{\em et al.,}}
\def\etalc{{\em et al.}} %for use in refs with collab name in ()s
\def\etc{{\em etc.}}
\def\ie{{\em i.e.,}}
\def\eg{{\em e.g.,}}
\def\vs{{\em vs.}}

\def\to{\rightarrow}
\def\ra{\rightarrow}


% Common combinations
\def\Bdk{$B$ decay}
\def\Bmeson{$B$ meson}
\def\Bmesons{$B$ mesons}
\def\daq{data acquisition}

% Stuff for bibliographies:
% BaBar notes:
\newcommand{\babarnote}[1] {\mbox{\babar\ {\sl Note}~\# #1}}
\newcommand{\babarnoteup}[1] {\mbox{\babar\ Note~\# #1}}
% Letter of intent and Conc. Design Report (for PEP-II)
\def\LOI{{\sl Letter of Intent}}
\def\CDR{{\sl Conceptual Design Report}}
\def\TDR{{\sl Technical Design Report}}

%% Units not in babarsym.tex
% Time-Frequency
\def\hz	  {\ensuremath{\mbox{\,Hz}}}
\def\khz  {\ensuremath{\mbox{\,kHz}}}
\def\mhz  {\ensuremath{\mbox{\,MHz}}}
\def\ghz  {\ensuremath{\mbox{\,GHz}}}
% Electrical
\def\muv  	{\ensuremath{\mbox{\,$\mu$V}}}
\def\mv  	{\ensuremath{\mbox{\,mV}}}
\def\volt  	{\ensuremath{\mbox{\,V}}}
\def\kv  	{\ensuremath{\mbox{\,kV}}}
\def\mw  	{\ensuremath{\mbox{\,mW}}}
\def\kw  	{\ensuremath{\mbox{\,kW}}}
\def\watt  	{\ensuremath{\mbox{\,W}}}
\def\ohm  	{\ensuremath{\mbox{\,$\Omega$}}}
\def\Mohm  	{\ensuremath{\mbox{\,M$\Omega$}}}
\def\mohm       {\ensuremath{\mbox{\,m$\Omega$}}}
\def\kohm       {\ensuremath{\mbox{\,k$\Omega$}}}
\def\kA         {\ensuremath{\mbox{\,kA}}}
\def\Amp        {\ensuremath{\mbox{\,A}}}
\def\mA         {\ensuremath{\mbox{\,mA}}}
\def\muA        {\ensuremath{\mbox{\,$\mu$A}}}
\def\nA         {\ensuremath{\mbox{\,nA}}}
\def\Coul       {\ensuremath{\mbox{\,C}}}
\def\fC         {\ensuremath{\mbox{\,fC}}}
\def\pf         {\ensuremath{\mbox{\,pF}}}
\def\nf         {\ensuremath{\mbox{\,nF}}}
% Pressure
\def\ntorr      {\ensuremath{\mbox{\,nTorr}}}
\def\mbar       {\ensuremath{\mbox{\,mbar}}}
\def\kpa        {\ensuremath{\mbox{\,kPa}}}
\def\mpa        {\ensuremath{\mbox{\,MPa}}}
% Force
\def\MN         {\ensuremath{\mbox{\,MN}}}
\def\kN         {\ensuremath{\mbox{\,kN}}}
% Misc
\def\kg   {\ensuremath{\,\mbox{kg}}}
\def\liter{\ensuremath{\,\ell}}
\def\dF   {\ensuremath{\mbox{\degrees F}}}
\def\tesla{\ensuremath{\mbox{\,T}}}
\def\mtesla{\ensuremath{\mbox{\,mT}}}
%
% The following definition for milli-radian overrides that in the Official BABAR PubBoard
% symbol definition table.  
% milliradian will be expressed as mrad
% radiation (rads) is a deprecated unit but will be used in preference to cGy (centiGray);
% the symbol in the paper will be Rad (and mRad, kRad, MRad, etc.)
% [Requested by Vera Luth, 11 Jan 2001]
\def\mrad       {\ensuremath{\mbox{\,mrad}}}
%
% The following definition for Pt (transverse momentum) overrides that in the Official BABAR 
% PubBoard symbol def table.  Instead of p_T, use p_t (change upper case T to lower case).
% [Requested by Vera Luth, 23 Jan 2001]
%\def\pxy        {\ensuremath{\mbox{p_{\rm t}}}}  %this does not work!
%\def\pt         {\ensuremath{\mbox{p_{\rm t}}}}  %nor does this!
\def\pxy        {\mbox{$p_{\rm t}$}}
%\def\pxy        {\mbox{$p_T$}}
\def\pt         {\mbox{$p_{\rm t}$}}
%\def\pt         {\mbox{$p_T$}}

% Requested 6 March 2000 by VGL
%\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}}
\renewcommand{\dedx}{\ensuremath{dE/dx}}


==> authors.tex <==
\begin{center}
\small

\long\def\inst#1{\par\nobreak\kern 4pt\nobreak
    {\it #1}\par\vskip 10pt plus 3pt minus 3pt}

The \babar\ Collaboration
\bigskip

%% author list as of 02-Nov-2000 (712 authors)
B.~Aubert,
A.~Bazan,
A.~Boucham,
D.~Boutigny,
I.~De Bonis,
J.~Favier,
J.-M.~Gaillard,
A.~Jeremie,
Y.~Karyotakis,
T.~Le Flour,
J.P.~Lees,
S.~Lieunard,
P.~Petitpas,
P.~Robbe,
V.~Tisserand,
K.~Zachariadou
\inst{Laboratoire de Physique des Particules, F-74941 Annecy-le-Vieux, France }
A.~Palano
\inst{Universit\`a di Bari, Dipartimento di Fisica and INFN, I-70126 Bari, Italy }
G.P.~Chen,
J.C.~Chen,
N.D.~Qi,
G.~Rong,
P.~Wang,
Y.S.~Zhu
\inst{Institute of High Energy Physics, Beijing 100039, China }
G.~Eigen,
P.L.~Reinertsen,
B.~Stugu
\inst{University of Bergen, N-5007 Bergen, Norway }
B.~Abbott,
G.S.~Abrams,
L.~Amerman,
A.W.~Borgland,
A.B.~Breon,
D.N.~Brown,
J.~Button-Shafer,
A.R.~Clark,
S.~Dardin,
C.~Day,
S.F.~Dow,
Q.~Fan,
I.~Gaponenko,
M.S.~Gill,
F.R.~Goozen,
S.J.~Gowdy,
A.~Gritsan,
Y.~Groysman,
C.~Hernikl,
R.G.~Jacobsen,
R.C.~Jared,
R.W.~Kadel,
J.~Kadyk,
A.~Karcher,
L.T.~Kerth,
I.~Kipnis,
S.~Kluth,
J.F.~Kral,
R.~Lafever,
C.~LeClerc,
M.E.~Levi,
S.A.~Lewis,
C.~Lionberger,
T.~Liu,
M.~Long,
L.~Luo,
G.~Lynch,
P.~Luft,
E.~Mandelli,
M.~Marino,
K.~Marks,
C.~Matuk,
A.B.~Meyer,
R.~Minor,
A.~Mokhtarani,
M.~Momayezi,
M.~Nyman,
P.J.~Oddone,
J.~Ohnemus,
D.~Oshatz,
S.~Patton,
M.~Pedrali-Noy,
A.~Perazzo,
C.~Peters,
W.~Pope,
M.~Pripstein,
D.R.~Quarrie,
J.E.~Rasson,
N.A.~Roe,
A.~Romosan,
M.T.~Ronan,
V.G.~Shelkov,
R.~Stone,
P.D.~Strother,\footnote{Now at Queen Mary, University of London, London, E1 4NS, UK}
A.V.~Telnov,
H.~von der Lippe,
T.F.~Weber,
W.A.~Wenzel,
G.~Zizka
\inst{Lawrence Berkeley National Laboratory and University of California, Berkeley, CA 94720, USA }
P.G.~Bright-Thomas,
C.M.~Hawkes,
A.~Kirk,
D.~J.~Knowles,
S.W.~O'Neale,
A.T.~Watson,
N.K.~Watson
\inst{University of Birmingham, Birmingham, B15 2TT, UK }
T.~Deppermann,
H.~Koch,
J.~Krug,
M.~Kunze,
B.~Lewandowski,
K.~Peters,
H.~Schmuecker,
M.~Steinke
\inst{Ruhr Universit\"at Bochum, Inst.\ f.\ Experimentalphysik 1, D-44780 Bochum, Germany }
J.C.~Andress,
N.R.~Barlow,
W.~Bhimji,
N.~Chevalier,
P.J.~Clark,
W.N.~Cottingham,
N.~De Groot,
N.~Dyce,
B.~Foster,
A.~Mass,
J.D.~McFall,
D.~Wallom,
F.F.~Wilson
\inst{University of Bristol, Bristol BS8 1TL, UK }
K.~Abe,
C.~Hearty,
J.A.~McKenna,
D.~Thiessen
\inst{University of British Columbia, Vancouver, BC, Canada V6T 1Z1 }
B.~Camanzi,
T.J.~Harrison,\footnote{Now at University of Birmingham, Birmingham B15 2TT, UK}
A.K.~McKemey,
J.~Tinslay
\inst{Brunel University, Uxbridge, Middlesex UB8 3PH, UK }
E.I.~Antohin,
V.E.~Blinov,
A.D.~Bukin,
D.A.~Bukin,
A.R.~Buzykaev,
M.S.~Dubrovin,
V.B.~Golubev,
V.N.~Ivanchenko,
G.M.~Kolachev,
A.A.~Korol,
E.A.~Kravchenko,
S.F.~Mikhailov,
A.P.~Onuchin,
A.A.~Salnikov,
S.I.~Serednyakov,
Yu.I.~Skovpen,
V.I.~Telnov,
A.N.~Yushkov
\inst{Budker Institute of Nuclear Physics, Novosibirsk 630090, Russia }
J.~Booth,
A.J.~Lankford,
M.~Mandelkern,
S.~Pier,
D.P.~Stoker,
G.~Zioulas
\inst{University of California at Irvine, Irvine, CA 92697, USA }
A.~Ahsan,
K.~Arisaka,
C.~Buchanan,
S.~Chun
\inst{University of California at Los Angeles, Los Angeles, CA 90024, USA }
R.~Faccini,\footnote{Jointly appointed with Universit\`a di Roma La Sapienza, Dipartimento di Fisica and INFN, I-00185 Roma, Italy}
D.B.~MacFarlane,
S.A.~Prell,
Sh.~Rahatlou,
G.~Raven,
V.~Sharma
\inst{University of California at San Diego, La Jolla, CA 92093, USA }
S.~Burke,
D.~Callahan,
C.~Campagnari,
B.~Dahmes,
D.~Hale,
P.A.~Hart,
N.~Kuznetsova,
S.~Kyre,
S.~L.~Levy,
O.~Long,
A.~Lu,
J.~May,
J.D.~Richman,
W.~Verkerke,
M.~Witherell,
S.~Yellin
\inst{University of California at Santa Barbara, Santa Barbara, CA 93106, USA }
J.~Beringer,
J.~DeWitt,
D.E.~Dorfan,
A.M.~Eisner,
A.~Frey,
A.A.~Grillo,
M.~Grothe,
C.A.~Heusch,
R.P.~Johnson,
W.~Kroeger,
W.S.~Lockman,
T.~Pulliam,
W.~Rowe,
H.~Sadrozinski,
T.~Schalk,
R.E.~Schmitz,
B.A.~Schumm,
A.~Seiden,
E.N.~Spencer,
M.~Turri,
W.~Walkowiak,
M.~Wilder,
D.C.~Williams
\inst{University of California at Santa Cruz, Santa Cruz, CA 95064, USA }
E.~Chen,
G.P.~Dubois-Felsmann,
A.~Dvoretskii,
J.E.~Hanson,
D.G.~Hitlin,
Yu.G.~Kolomensky,\footnote{Now at LBNL and University of California, Berkeley, CA 94720, USA}
S.~Metzler,
J.~Oyang,
F.C.~Porter,
A.~Ryd,
A.~Samuel,
M.~Weaver,
S.~Yang,
R.Y.~Zhu
\inst{California Institute of Technology, Pasadena, CA 91125, USA }
S.~Devmal,
T.L.~Geld,
S.~Jayatilleke,
S.M.~Jayatilleke,
G.~Mancinelli,
B.T.~Meadows,
M.D.~Sokoloff
\inst{University of Cincinnati, Cincinnati, OH 45221, USA }
P.~Bloom,
B.~Broomer,
E.~Erdos,
S.~Fahey,
W.T.~Ford,
F.~Gaede,
W.C.~van Hoek,
D.R.~Johnson,
A.K.~Michael,
U.~Nauenberg,
A.~Olivas,
H.~Park,
P.~Rankin,
J.~Roy,
S.~Sen,
J.G.~Smith,
D.L.~Wagner
\inst{University of Colorado, Boulder, CO 80309, USA }
J.~Blouw,
J.L.~Harton,
M.~Krishnamurthy,
A.~Soffer,
W.H.~Toki,
D.W.~Warner,
R.J.~Wilson,
J.~Zhang
\inst{Colorado State University, Fort Collins, CO 80523, USA }
T.~Brandt,
J.~Brose,
G.~Dahlinger,
M.~Dickopp,
R.S.~Dubitzky,
P.~Eckstein,
H.~Futterschneider,
M.L.~Kocian,
R.~Krause,
R.~M\"uller-Pfefferkorn,
K.R.~Schubert,
R.~Schwierz,
B.~Spaan,
L.~Wilden
\inst{Technische Universit\"at Dresden, D-01062 Dresden, Germany }
L.~Behr,
D.~Bernard,
G.R.~Bonneaud,
F.~Brochard,
J.~Cohen-Tanugi,
S.~Ferrag,
G.~Fouque,
F.~Gastaldi,
P.~Matricon,
P.~Mora de Freitas,
C.~Renard,
E.~Roussot,
S.~T'Jampens,
C.~Thiebaux,
G.~Vasileiadis,
M.~Verderi
\inst{Ecole Polytechnique, F-91128 Palaiseau, France }
A.~Anjomshoaa,
R.~Bernet,
F.~Di Lodovico,
F.~Muheim,
S.~Playfer,
J.E.~Swain
\inst{University of Edinburgh, Edinburgh EH9 3JZ, UK }
M.~Falbo
\inst{Elon College, Elon College, NC 27244, USA}
C.~Bozzi,
S.~Dittongo,
M.~Folegani,
L.~Piemontese,
A..C.~Ramusino
\inst{Universit\`a di Ferrara, Dipartimento di Fisica and INFN, I-44100 Ferrara, Italy }
E.~Treadwell
\inst{Florida A\&M University, Tallahassee, FL 32307, USA }
F.~Anulli,\footnote{Jointly appointed with Univ.\ di Perugia, I-06100 Perugia, Italy}
R.~Baldini-Ferroli,
A.~Calcaterra,
R.~de Sangro,
D.~Falciai,
G.~Finocchiaro,
P.~Patteri,
I.M.~Peruzzi,\footnotemark[5]
M.~Piccolo,
Y.~Xie,
A.~Zallo
\inst{Laboratori Nazionali di Frascati dell'INFN, I-00044 Frascati, Italy }
S.~Bagnasco,
A.~Buzzo,
R.~Contri,
G.~Crosetti,
P.~Fabbricatore,
S.~Farinon,
M.~Lo Vetere,
M.~Macri,
S.~Minutoli,
M.R.~Monge,
R.~Musenich,
M.~Pallavicini,
R.~Parodi,
S.~Passaggio,
F.C.~Pastore,
C.~Patrignani,
M.G.~Pia,
C.~Priano,
E.~Robutti,
A.~Santroni
\inst{Universit\`a di Genova, Dipartimento di Fisica and INFN, I-16146 Genova, Italy }
R.~Bartoldus,
T.~Dignan,
R.~Hamilton,
U.~Mallik
\inst{University of Iowa, Iowa City, IA 52242, USA }
J.~Cochran,
H.B.~Crawley,
P.A.~Fischer,
J.~Lamsa,
R.~McKay,
W.T.~Meyer,
E.I.~Rosenberg
\inst{Iowa State University, Ames, IA 50011-3160, USA }
J.N.~Albert,
C.~Beigbeder,
M.~Benkebil,
D.~Breton,
R.~Cizeron,
S.~Du,
G.~Grosdidier,
C.~Hast,
A.~H\"ocker,
H.~M.~Lacker,
V.~LePeltier,
A.M.~Lutz,
S.~Plaszczynski,
M.H.~Schune,
S.~Trincaz-Duvoid,
K.~Truong,
A.~Valassi,
G.~Wormser
\inst{Laboratoire de l'Acc\'el\'erateur Lin\'eaire, F-91898 Orsay, France }
O.~Alford,
D.~Behne,
R.M.~Bionta,
J.~Bowman,
V.~Brigljevi\'c,
A.~Brooks,
V.A.~Dacosta,
O.~Fackler,
D.~Fujino,
M.~Harper,
D.J.~Lange,
M.~Mugge,
T.G.~O'Connor,
H.~Olson,
L.~Ott,
E.~Parker,
B.~Pedrotti,
M.~Roeben,
X.~Shi,
K.~van Bibber,
T.J.~Wenaus,
D.M.~Wright,
C.R.~Wuest,
B.~Yamamoto
\inst{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA }
M.~Carroll,
P.~Cooke,
J.R.~Fry,
E.~Gabathuler,
R.~Gamet,
M.~George,
M.~Kay,
S.~McMahon,\footnote{Now at University of California at Irvine, Irvine, CA 92697, USA}
A.~Muir,
D.J.~Payne,
R.J.~Sloane,
P.~Sutcliffe,
C.~Touramanis
\inst{University of Liverpool, Liverpool L69 3BX, UK }
M.L.~Aspinwall,
D.A.~Bowerman,
P.D.~Dauncey,
I.~Eschrich,
N.J.W.~Gunawardane,
R.~Martin,
J.A.~Nash,
D.R.~Price,
P.Sanders,
D.Smith
\inst{University of London, Imperial College, London, SW7 2BW, UK }
D.E.~Azzopardi,
J.J.~Back,
P.~Dixon,
P.F.~Harrison,
D.~Newman-Coburn,\footnote{Deceased}
R.J.L.~Potter,
H.W.~Shorthouse,
M.I.~Williams,
P.B.~Vidal
\inst{Queen Mary, University of London, London, E1 4NS, UK }
G.~Cowan,
S.~George,
M.G.~Green,
A.~Kurup,
C.E.~Marker,
P.~McGrath,
T.R.~McMahon,
F.~Salvatore,
I.~Scott,
G.~Vaitsas
\inst{University of London, Royal Holloway and Bedford New College, Egham, Surrey TW20 0EX, UK }
D.~Brown,
C.~L.~Davis,
Y.~Li,
J.~Pavlovich
\inst{University of Louisville, Louisville, KY 40292, USA }
J.~Allison,
R.J.~Barlow,
J.T.~Boyd,
J.~Fullwood,
F.~Jackson,
A.~Khan,\footnote{Now at University of Edinburgh, Edinburgh EH9 3JZ, UK}
G.D.~Lafferty,
N.~Savvas,
E.T.~Simopoulos,
R.J.~Thompson,
J.H.~Weatherall
\inst{University of Manchester, Manchester M13 9PL, UK }
R.~Bard,
C.~Dallapiccola,\footnote{Now at University of Massachusetts, Amherst, MA 01003, USA}
A.~Farbin,
A.~Jawahery,
V.~Lillard,
J.~Olsen,
D.A.~Roberts,
J.R.~Schieck
\inst{University of Maryland, College Park, MD 20742, USA }
G.~Blaylock,
K.T.~Flood,
S.S.~Hertzbach,
R.~Kofler,
C.S.~Lin,
S.~Willocq,
J.~Wittlin
\inst{University of Massachusetts, Amherst, MA 01003, USA }
B.~Brau,
R.~Cowan,
F.~Taylor,
R.K.~Yamamoto
\inst{Massachusetts Institute of Technology, Cambridge, MA 02139, USA }
D.I.~Britton,
R.~Fernholz,\footnote{Now at Princeton University, Princeton, NJ 08544, USA}
M.~Houde,
M.~Milek,
P.M.~Patel,
J.~Trischuk
\inst{McGill University, Montr\'eal, QC, Canada H3A 2T8 }
F.~Lanni,
F.~Palombo
\inst{Universit\`a di Milano, Dipartimento di Fisica and INFN, I-20133 Milano, Italy }
J.M.~Bauer,
M.~Booke,
L.~Cremaldi,
R.~Kroeger,
M.~Reep,
J.~Reidy,
D.A.~Sanders,
D.J.~Summers
\inst{University of Mississippi, University, MS 38677, USA }
J.~F.~Arguin,
M.~Beaulieu,
J.~P.~Martin,
J.~Y.~Nief,
R.~Seitz,
P.~Taras,
A.~Woch,
V.~Zacek
\inst{Universit\'e de Montr\'eal, Lab.\ Ren\'e J.A.~L\'evesque, Montr\'eal, QC, Canada, H3C 3J7 }
H.~Nicholson,
C.S.~Sutton
\inst{Mount Holyoke College, South Hadley, MA 01075, USA }
C.~Cartero,
N.~Cavallo,\footnote{Also with Universit\`a della Basilicata, I-85100 Portenza, Italy }
G.~De Nardo,
F.~Fabozzi,
C.~Gatto,
L.~Lista,
D.~Piccolo,
C.~Sciacca
\inst{Universit\`a di Napoli Federico II, Dipartimento di Fisica and INFN, I-80126 Napoli, Italy }
N.~M.~Cason, J.~M.~LoSecco
\inst{University of Notre Dame, Notre Dame, IN 46556, USA }
J.R.~G.~Alsmiller,
T.A.~Gabriel,
T.~Handler,
J.~Heck
\inst{Oak Ridge National Laboratory, Oak Ridge, TN 37831, USA }
M.~Iwasaki,
N.B.~Sinev,
\inst{University of Oregon, Eugene, OR 97403, USA }
R.~Caracciolo,
F.~Colecchia,
F.~Dal Corso,
F.~Galeazzi,
M.~Marzolla,
G.~Michelon,
M.~Morandin,
M.~Posocco,
M.~Rotondo,
S.~Santi,
F.~Simonetto,
R.~Stroili,
E.~Torassa,
C.~Voci
\inst{Universit\`a di Padova, Dipartimento di Fisica and INFN, I-35131 Padova, Italy }
P.~Bailly,
M.~Benayoun,
H.~Briand,
J.~Chauveau,
P.~David,
C.~De la Vaissi\`ere,
L.~Del Buono,
J.-F.~Genat,
O.~Hamon,
Ph.~Leruste,
F.~Le Diberder,
H.~Lebbolo,
J.~Lory,
L.~Martin,
F.~Martinez-Vidal,\footnote{Now at Universit\`a di Pisa, I-56010 Pisa, Italy }
L.~Roos,
J.~Stark,
S.~Versill\'e,
B.~Zhang
\inst{Universit\'e Paris VI et VII, F-75252 Paris, France }
P.F.~Manfredi,
L.~Ratti,
V.~Re,
V.~Speziali
\inst{Universit\`a di Pavia, Dipartimento di Fisica and INFN, I-27100 Pavia, Italy }
E.D.~Frank,
L.~Gladney,
Q.H.~Guo,
J.H.~Panetta
\inst{University of Pennsylvania, Philadelphia, PA 19104, USA }
C.~Angelini,
G.~Batignani,
S.~Bettarini,
M.~Bondioli,
F.~Bosi,
M.~Carpinelli,
F.~Forti,
A.~Gaddi,
D.~Gagliardi,
M.A.~Giorgi,
A.~Lusiani,
P.~Mammini,
M.~Morganti,
F.~Morsani,
N.~Neri,
A.~Profeti,
E.~Paoloni,
F.~Raffaelli,
M.~Rama,
G.~Rizzo,
F.~Sandrelli,
G.~Simi,
G.~Triggiani
\inst{Universit\`a di Pisa, Scuola Normale Superiore, and INFN, I-56010 Pisa, Italy }
M.~Haire,
D.~Judd,
K.~Paick,
L.~Turnbull,
D.~E.~Wagoner
\inst{Prairie View A\&M University, Prairie View, TX 77446, USA }
J.~Albert,
C.~Bula,
M.H.~Kelsey,
C.~Lu,
K.T.~McDonald,
V.~Miftakov,
B.~Sands,
S.F.~Schaffner,
A.J.S.~Smith,
A.~Tumanov,
E.W.~Varnes
\inst{Princeton University, Princeton, NJ 08544, USA }
F.~Bronzini,
A.~Buccheri,
C.~Bulfon,
G.~Cavoto,
D.~del Re,
F.~Ferrarotto,
F.~Ferroni,
K.~Fratini,
E.~Lamanna,
E.~Leonardi,
M.A.~Mazzoni,
S.~Morganti,
G.~Piredda,
F.~Safai Tehrani,
M.~Serra,
C.~Voena
\inst{Universit\`a di Roma La Sapienza, Dipartimento di Fisica and INFN, I-00185 Roma, Italy }
R.~Waldi
\inst{Universit\"at Rostock, D-18051 Rostock, Germany }
P.F.~Jacques,
M.~Kalelkar,
R.J.~Plano
\inst{Rutgers University, New Brunswick, NJ 08903, USA }
T.~Adye,
B.~Claxton,
J.~Dowdell,
U.~Egede,
B.~Franek,
S.~Galagedera,
N.I.~Geddes,
G.P.~Gopal,
J.~Kay,\footnote{At CLRC Daresbury Laboratory, Daresbury, Warrington, Cheshire, WA4 4AD, UK}
J.~Lidbury,
S.~Madani,
S.~Metcalfe,\footnotemark[13]$^,$\footnote{Now at Stanford Linear Accelerator Center, Stanford, CA 94309, USA}
G.~Markey,\footnotemark[13]
P.~Olley,
M.~Watt,
S.M.~Xella
\inst{Rutherford Appleton Laboratory, Didcot, Oxon., OX11 0QX, UK}
R.~Aleksan,
P.~Besson,\footnotemark[7]
P.~Bourgeois,
P.~Convert,
G.~De Domenico,
A.~de Lesquen,
S.~Emery,
A.~Gaidot,
S.~F.~Ganzhur,
Z.~Georgette,
L.~Gosset,
P.~Graffin,
G.~Hamel de Monchenault,
S.~Herv\' e,
M.~Karolak,
W.~Kozanecki,
M.~Langer,
G.W.~London,
V.~Marques,
B.~Mayer,
P.~Micout,
J.P.~Mols,
J.P.~Mouly,
Y.~Penichot,
J.~Rolquin,
B.~Serfass,
J.C.~Toussaint,
M.~Usseglio,
G.~Vasseur,
C.~Yeche,
M.~Zito
\inst{DAPNIA, Commissariat \`a l'Energie Atomique/Saclay, F-91191 Gif-sur-Yvette, France }
N.~Copty,
M.V.~Purohit,
F.X.~Yumiceva
\inst{University of South Carolina, Columbia, SC 29208, USA }
I.~Adam,
A.~Adesanya,
P.L.~Anthony,
D.~Aston,
J.~Bartelt,
J.~Becla,
R.~Bell,
E.~Bloom,
C.T.~Boeheim,
A.M.~Boyarski,
R.F.~Boyce,
D.~Briggs,
F.~Bulos,
W.~Burgess,
B.~Byers,
G.~Calderini,
R.~Chestnut,
R.~Claus,
M.R.~Convery,
R.~Coombes,
L.~Cottrell,
D.P.~Coupal,
D.H.~Coward,
W.W.~Craddock,
S.~DeBarger,
H.~DeStaebler,
J.~Dorfan,
M.~Doser,
W.~Dunwoodie,
J.E.~Dusatko,
S.~Ecklund,
T.H.~Fieguth,
D.R.~Freytag,
T.~Glanzman,
G.L.~Godfrey,
G.~Haller,
A.~Hanushevsky,
J.~Harris,
A.~Hasan,
C.~Hee,
T.~Himel,
M.E.~Huffer,
T.~Hung,
W.R.~Innes,
C.P.~Jessop,
H.~Kawahara,
L.~Keller,
M.E.~King,
L.~Klaisner,
H.J.~Krebs,
U.~Langenegger,
W.~Langeveld,
D.W.G.S.~Leith,
S.K.~Louie,
S.~Luitz,
V.~Luth,
H.L.~Lynch,
J.~McDonald,
G.~Manzin,
H.~Marsiske,
T.~Mattison,\footnote{Now at University of British Columbia, Vancouver, BC, Canada V6T 1Z1}
M.~McCulloch,
M.~McDougald,
D.~McShurley,
S.~Menke,
R.~Messner,
S.~Metcalfe,
M.~Morii,\footnote{Now at Harvard University, Cambridge, MA 02138}
R.~Mount,
D.~R.~Muller,
D.~Nelson,
M.~Norby,
C.P.~O'Grady,
L.~Olavson,
J.~Olsen,
F.G.~O'Neill,
G.~Oxoby,
P.~Paolucci,\footnote{Now at Universit\`a di Napoli Federico II, I-80126 Napoli, Italy}
T.~Pavel,
J.~Perl,
M.~Pertsova,
S.~Petrak,
G.~Putallaz,
P.E.~Raines,
B.N.~Ratcliff,
R.~Reif,
S.H.~Robertson,
L.S.~Rochester,
A.~Roodman,
J.J.~Russel,
L.~Sapozhnikov,
O.H.~Saxton,
T.~Schietinger,
R.H.~Schindler,
J.~Schwiening,
G.~Sciolla,\footnote{Now at Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
J.T.~Seeman,
V.V.~Serbo,
S.~Shapiro,
K.~Skarpass Sr.,
A.~Snyder,
E.~Soderstrom,
A.~Soha,
S.M.~Spanier,
A.~Stahl,
P.~Stiles,
D.~Su,
M.K.~Sullivan,
M.~Talby,
H.A.~Tanaka,
J.~Va'vra,
S.R.~Wagner,
R.~Wang,
T.~Weber,
A.J.R.~Weinstein,
J.L.~White,
U.~Wienands,
W.J.~Wisniewski,
C.C.~Young,
N.~Yu
\inst{Stanford Linear Accelerator Center, Stanford, CA 94309, USA }
P.R.~Burchat,
C.H.~Cheng,
D.~Kirkby,
T.I.~Meyer,
C.~Roat
\inst{Stanford University, Stanford, CA 94305-4060, USA }
R.~Henderson,
N.~Khan
\inst{TRIUMF, Vancouver, BC, Canada V6T 2A3 }
S.~Berridge,
W.~Bugg,
H.~Cohn,
E.~Hart,
A.W.~Weidemann
\inst{University of Tennessee, Knoxville, TN 37996, USA }
T.~Benninger,
J.M.~Izen,
I.~Kitayama,
X.C.~Lou,
M.~Turcotte
\inst{University of Texas at Dallas, Richardson, TX 75083, USA }
F.~Bianchi,
M.~Bona,
F.~Daudo,
B.~Di Girolamo,
D.~Gamba,
P.~Grosso,
A.~Smol,
P..P.~Trapani,
D.~Zanin
\inst{Universit\`a di Torino, Dipartimento di Fisica and INFN, I-10125 Torino, Italy }
L.~Bosisio,
G.~Della Ricca,
L.~Lanceri,
A.~Pompili,
P.~Poropat,
M.~Prest,
I.~Rashevskaia,
E.~Vallazza,
G.~Vuagnin
\inst{Universit\`a di Trieste, Dipartimento di Fisica and INFN, I-34127 Trieste, Italy }
R.S.~Panvini
\inst{Vanderbilt University, Nashville, TN 37235, USA }
C.~Brown,
A.~De Silva,\footnote{Now at TRIUMF, Vancouver, BC, Canada V6T 2A3}
R.~Kowalewski,
D.~Pitman,
J.M.~Roney
\inst{University of Victoria, Victoria, BC, Canada V8W 3P6 }
H.R.~Band,
E.~Charles,
S.~Dasu,
P.~Elmer,
J.R.~Johnson,
J.~Nielsen,
W.~Orejudos,
Y.~Pan,
R.~Prepost,
I.J.~Scott,
J.~Walsh,\footnotemark[12]
S.L.~Wu,
Z.~Yu,
H.~Zobernig
\inst{University of Wisconsin, Madison, WI 53706, USA }
T.B.~Moore,
H.~Neal
\inst{Yale University, New Haven, CT 06511, USA }

\end{center}\newpage


==> babarsym_osaka2.tex <==
%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   11/14/00 D. MacFarlane  Corrected \kbyte macros for consistency
%%%%%   Revised    7/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised    7/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised    7/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised    7/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised    7/01/00 D. MacFarlane
%%%%%   Revised    6/21/00 D. Hitlin
%%%%%   Original   6/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}}
\def\en         {\ensuremath{e^-}}      % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}}
\def\epm        {\ensuremath{e^\pm}}
\def\epem       {\ensuremath{e^+e^-}}
\def\ee         {\ensuremath{e^-e^-}}
\def\mmu        {\ensuremath{\mu}}
\def\mup        {\ensuremath{\mu^+}}
\def\mun        {\ensuremath{\mu^-}}    % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}}
\def\mtau       {\ensuremath{\tau}}
\def\taup       {\ensuremath{\tau^+}}
\def\taum       {\ensuremath{\tau^-}}
\def\tautau     {\ensuremath{\tau^+\tau^-}}
\def\ellm       {\ensuremath{\ell^-}}
\def\ellp       {\ensuremath{\ell^+}}
\def\ellell     {\ensuremath{\ell^+ \ell^-}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}}
\def\gaga  {\ensuremath{\gamma\gamma}}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%  LEPTONS & PHOTONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ega   {\ensuremath{e\gamma}}
\def\game  {\ensuremath{\gamma e^-}}
\def\epemg  {\ensuremath{e^+e^-\gamma}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q   {\ensuremath{q}}
\def\qbar  {\ensuremath{\overline q}}
\def\qqbar {\ensuremath{q\overline q}}
\def\u  {\ensuremath{u}}
\def\ubar  {\ensuremath{\overline u}}
\def\uubar {\ensuremath{u\overline u}}
\def\d  {\ensuremath{d}}
\def\dbar  {\ensuremath{\overline d}}
\def\ddbar {\ensuremath{d\overline d}}
\def\s  {\ensuremath{s}}
\def\sbar  {\ensuremath{\overline s}}
\def\ssbar {\ensuremath{s\overline s}}
\def\c  {\ensuremath{c}}
\def\cbar  {\ensuremath{\overline c}}
\def\ccbar {\ensuremath{c\overline c}}
\def\b  {\ensuremath{b}}
\def\bbar  {\ensuremath{\overline b}}
\def\bbbar {\ensuremath{b\overline b}}
\def\t  {\ensuremath{t}}
\def\tbar  {\ensuremath{\overline t}}
\def\tbar  {\ensuremath{\overline t}}
\def\ttbar {\ensuremath{t\overline t}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   HADRONS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}}
\def\ppz   {\ensuremath{\pi^0\pi^0}}
\def\pip   {\ensuremath{\pi^+}}
\def\pim   {\ensuremath{\pi^-}}
\def\pipi  {\ensuremath{\pi^+\pi^-}}
\def\pipm   {\ensuremath{\pi^\pm}}
\def\pimp   {\ensuremath{\pi^\mp}}
\def\kaon  {\ensuremath{K}}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}}
\def\Kb    {\ensuremath{\Kbar}}
\def\Kpm   {\ensuremath{K^\pm}}
\def\Kp    {\ensuremath{K^+}}
\def\Km    {\ensuremath{K^-}}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}}
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}}
\def\Kstarz  {\ensuremath{K^{*0}}}
\def\Kstarzb  {\ensuremath{\Kbar^{*0}}}
\def\Kstar   {\ensuremath{K^*}}
\def\Kstarb  {\ensuremath{\Kbar^*}}
\def\Kstarp   {\ensuremath{K^{*+}}}
\def\Kstarm   {\ensuremath{K^{*-}}}
\def\Kstarpm   {\ensuremath{K^{*\pm}}}
\def\Kzb   {\ensuremath{\Kbar^0}}
\def\KzKzb {\ensuremath{K^0 \kern -0.16em \Kzb}}
\def\Dz    {\ensuremath{D^0}}
%%% do NOT use ensuremath here
\def\Dbar  {\kern 0.2em\overline{\kern -0.2em D}{}}
\def\Db    {\ensuremath{\Dbar}}
\def\Dzb   {\ensuremath{\Dbar^0}}
\def\DzDzb {\ensuremath{D^0 {\kern -0.16em \Dzb}}}
\def\Dstar   {\ensuremath{D^*}}
\def\Dstarb   {\ensuremath{\Dbar^*}}
\def\Dstarz  {\ensuremath{D^{*0}}}
\def\Dstarzb  {\ensuremath{\Dbar^{*0}}}
\def\Ds    {\ensuremath{D^+_s}}
\def\Dsb   {\ensuremath{\Dbar^+_s}}
\def\Dss   {\ensuremath{D^*_s}}
\def\Bz    {\ensuremath{B^0}}
\def\B     {\ensuremath{B}}
%%% do NOT use ensuremath here
\def\Bbar  {\kern 0.18em\overline{\kern -0.18em B}{}}
\def\Bb    {\ensuremath{\Bbar}}
\def\Bzb   {\ensuremath{\Bbar^0}}
\def\Bu    {\ensuremath{B^+}}
\def\Bub   {\ensuremath{B^-}}
\def\Bpm   {\ensuremath{B^\pm}}
\def\Bs    {\ensuremath{B_s}}
\def\Bsb   {\ensuremath{\Bbar_s}}
\def\BB    {\ensuremath{B\Bbar}}
\def\BzBzb {\ensuremath{B^0 {\kern -0.16em \Bzb}}}

\def\jpsi  {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}}
%\def\psitwos {\ensuremath{\psi{\rm (2S)}}} % dbm: conform to PDG
\def\psitwos {\ensuremath{\psi{(2S)}}}
%\def\psip {\ensuremath{\psi^{\prime}}}
\mathchardef\Upsilon="7107
%\def\Y#1S{\ensuremath{\Upsilon{\rm(#1S)}}}% no space before {...}! dbm: conform to PDG
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\Xpart {\ensuremath{X}}

\def\proton     {\ensuremath{p}}
\def\antiproton {\ensuremath{\overline p}}
\def\neutron    {\ensuremath{n}}
\def\antineutron  {\ensuremath{\overline n}}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A
%%% do NOT use ensuremath here
\def\Deltabar   {\kern 0.25em\overline{\kern -0.25em \Deltares}{}}
\def\Lbar {\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}}
\def\Xbar{\kern 0.2em\overline{\kern -0.2em X}{}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  BRANCHING RATIOS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR{{\ensuremath{\cal B}}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  REACTIONS    %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb {\ensuremath{\Upsilon{\rm( 4S)}\to B\Bbar}}
\def\upsbzbz {\ensuremath{\Upsilon{\rm( 4S)}\to\BzBzb}}
\def\upsbpbm {\ensuremath{\Upsilon{\rm( 4S)}\to\Bu\Bub}}
\def\bpsiks{\ensuremath{B^0 \to \jpsi \KS}}
\def\bpsikst{\ensuremath{B^0 \to \jpsi \Kstar}}
\def\bpsikl{\ensuremath{B^0 \to \jpsi \KL}}
\def\bpsikzeropi{\ensuremath{B^0 \to \jpsi (K^{*0} \to \KL\pi^0)}}
\def\bpsikpluspi{\ensuremath{B^+ \to \jpsi K^{*+},\ K^{*+} \to \KL\pi^+}}
\def\bpsikpluspi{\ensuremath{
{\Bz}/B^0 \to \jpsi ( \to \mu^+ \mu^-) K^{\pm} \pi^{\mp} }}
\def\bupsik{\ensuremath{B^{\pm} \to \jpsi ( \to \mu^+ \mu^-) K^{\pm} }}
\def\bpsiX{\ensuremath{B^0 \to \jpsi X}}
\def\upspsikl{\ensuremath{\FourS\to (\bpsikl) (\bzb \to X)}}
\def\Bzbtomu    {\ensuremath{\Bzb \to \mu {\rm X}}}
\def\Bzbtox     {\ensuremath{\Bzb \to {\rm X}}}
\def\Bztopipi   {\ensuremath{B^0 \to \pipi}}
\def\Bztokpi    {\ensuremath{B^0 \to K^{\pm}\pi^{\mp}}}
\def\Bztorhopi  {\ensuremath{B^0 \to \rho^+\pi^-}}
\def\Bztorhorho {\ensuremath{B^0 \to \rho\rho}}
\def\Bztokrho   {\ensuremath{B^0 \to K\rho}}
\def\Bztokstpi  {\ensuremath{B^0 \to \Kstar\pi}}
\def\Bztoapi    {\ensuremath{B^0 \to a_1\pi}}
\def\Bztodd     {\ensuremath{B^0 \to D^+D^-}}
\def\Bztodstd   {\ensuremath{B^0 \to D^{*+}D^-}}
\def\Bztodstdst {\ensuremath{B^0 \to D^{*+}D^{*-}}}
\def\BtoDK      {\ensuremath{B \to DK}}
\def\Btodstlnu  {\ensuremath{B \to D^*l\nu}}
\def\Btodstdlnu {\ensuremath{B \to D^*(D)l\nu}}
\def\Btorholnu  {\ensuremath{B \to \rho l\nu}}
\def\Btopilnu   {\ensuremath{B \to \pi l\nu}}
\def\Btoetah    {\ensuremath{B \to \eta h}}
\def\Btoetaph   {\ensuremath{B \to \eta ' h}}
\def\tauptoe    {\ensuremath{\taup \to \ep \nu \overline \nu}}
\def\taumtoe    {\ensuremath{\taum \to \en \nu \overline \nu}}
\def\tauptomu   {\ensuremath{\taup \to \mup \nu \overline \nu}}
\def\taumtomu    {\ensuremath{\taum \to \mun \nu \overline \nu}}
\def\Btoetaph   {\ensuremath{B \to \eta ' h}}
\def\tauptopi   {\ensuremath{\taup \to \pip \overline \nu}}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}}
\def\ggtopi     {\ensuremath{\gaga \to \pipi}}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}}
\def\ggstox     {\ensuremath{\ggstar \to \Xpart(1420) \to \kaon \kaon \pi}}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}}
\def\btosgam   {\ensuremath{b \to s \gamma}}
\def\btodgam   {\ensuremath{b \to d \gamma}}
\def\btosll    {\ensuremath{b \to s l^+l^-}}
\def\btosnunu   {\ensuremath{b \to s \nu\nu}}
\def\btosgaga   {\ensuremath{b \to s \gaga}}
\def\btosglue   {\ensuremath{b \to s g}}


% Kinematics

\def\ptot       {\mbox{$p$}}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}}
%\def\pt         {\mbox{$p_{\rm t}$}}
\def\pt         {\mbox{$p_T$}}
\def\mes        {\mbox{$m_{\rm ES}$}}
\def\mec        {\mbox{$m_{\rm EC}$}}


% Geometry
\def\mphi       {\mbox{$\phi$}}
\def\mtheta     {\mbox{$\theta$}}
\def\ctheta     {\mbox{$\cos \theta$}}

% UNITS
%
\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}}
\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}}
\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}}
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}}
\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}}
\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}}
\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}}
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}}
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}}
\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}}
\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}}
\def\syin {\ensuremath{^{\prime\prime}}}
\def\in   {\ensuremath{\rm \,in}}
\def\ft   {\ensuremath{\rm \,ft}}
\def\km   {\ensuremath{\rm \,km}}
\def\m    {\ensuremath{\rm \,m}}
\def\cm   {\ensuremath{\rm \,cm}}
\def\cma  {\ensuremath{{\rm \,cm}^2}}
\def\mm   {\ensuremath{\rm \,mm}}
\def\mma  {\ensuremath{{\rm \,mm}^2}}
%\def\mum  {\ensuremath{\rm \,\mum}}
\def\mum  {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma {\ensuremath{\rm \,\mum}^2}
\def\muma       {\ensuremath{\,\mu\rm m^2}}
\def\nm   {\ensuremath{\rm \,nm}}
\def\fm   {\ensuremath{\rm \,fm}}
%
\def\barn{\ensuremath{\rm \,b}}
\def\barnhyph{\ensuremath{\rm -b}}
\def\mbarn{\ensuremath{\rm \,mb}}
\def\mbarnhyph{\ensuremath{\rm -mb}}
\def\pb {\ensuremath{\rm \,pb}}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}}
\def\fb   {\ensuremath{\mbox{\,fb}}}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}}
%
\def\mus  {\ensuremath{\rm \,\mus}}
\def\ns   {\ensuremath{\rm \,ns}}
\def\ps   {\ensuremath{\rm \,ps}}
\def\fs   {\ensuremath{\rm \,fs}}
\def\gm   {\ensuremath{\rm \,g}}
%
\def\Xrad {\ensuremath{X_0}}
\def\NIL{\ensuremath{\lambda_{int}}}
\let\dgr\degrees

%
% Lengths / Areas
%
%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{\,\mathrm{cm}^{-2} \mathrm{s}^{-1}}}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}
%
\def\nm         {\ensuremath{\,\mathrm{nm}}}    %% nanometer
\def\nb         {\ensuremath{\,\mathrm{nb}}}
%%%%%
% Time
%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec        {\ensuremath{\,\mathrm{s}}}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{\,\mathrm{ms}}}      %% millisecond
\def\mus        {\ensuremath{\,\mu\mathrm{s}}}    %% microsecond
\def\ns         {\ensuremath{\,\mathrm{ns}}}      %% nanosecond
\def\ps         {\ensuremath{\,\mathrm{ps}}}   %% picosecond
%
% Data processing
\def\kbytes     {\ensuremath{\,\mathrm{kbytes}}}
\def\kbits      {\ensuremath{\,\mathrm{kbits}}}
\def\kbps       {\ensuremath{\,\mathrm{kbytes/s}}}
\def\kbsps      {\ensuremath{\,\mathrm{kbits/s}}}

\def\mbytes     {\ensuremath{\,\mathrm{Mbytes}}}
\def\mbits      {\ensuremath{\,\mathrm{Mbits}}}
\def\mbps       {\ensuremath{\,\mathrm{Mbytes/s}}}
\def\mbsps      {\ensuremath{\,\mathrm{Mbits/s}}}

\def\gbytes     {\ensuremath{\,\mathrm{Gbytes}}}
\def\gbits      {\ensuremath{\,\mathrm{Gbits}}}
\def\gbps       {\ensuremath{\,\mathrm{Gbytes/s}}}
\def\gbsps      {\ensuremath{\,\mathrm{Gbits/s}}}

\def\tbytes     {\ensuremath{\,\mathrm{Tbytes}}}
\def\tbits      {\ensuremath{\,\mathrm{Tbits}}}
\def\tbps       {\ensuremath{\,\mathrm{Tbytes/s}}}
\def\tbsps      {\ensuremath{\,\mathrm{Tbits/s}}}
\def\tbpy       {\ensuremath{\,\mathrm{Tbytes/yr}}}

% replaced by above consistent set: dbm, 11/14/00
%\def\kbytes     {\ensuremath{{\rm \,kbytes}}}
%\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}}
%\def\kbits      {\ensuremath{{\rm \,kbits}}}
%\def\kbsps      {\ensuremath{{\rm \,kbits/s}}}
%\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}}
%\def\mbytes     {\ensuremath{{\rm \,Mbytes}}}
%\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}}
%\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}}
%\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}}
%\def\gbytes     {\ensuremath{{\rm \,Gbytes}}}
%\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}}
%\def\tbytes     {\ensuremath{{\rm \,Tbytes}}}
%\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}}
%

\def\mic  {\ensuremath{\,\mu\mathrm{C}}}
\def\krad {\ensuremath{\,\mathrm{krad}}}
\def\cmc  {\ensuremath{\,\mathrm{cm}^3}}
\def\yr   {\ensuremath{\,\mathrm{yr}}}
\def\hr   {\ensuremath{\,\mathrm{hr}}}
\def\degc {\ensuremath{^\circ}{C}}
\def\degk {\ensuremath{\mathrm{K}}}
\def\degrees{\ensuremath{^{\circ}}}
\def\mrad{\ensuremath{\,\mathrm{mr}}}                %% milliradian
\def\mradhyph{\ensuremath{-\mathrm{mr}}}
%
\def\sx    {\ensuremath{\sigma_x}}
\def\sy    {\ensuremath{\sigma_y}}
\def\sz    {\ensuremath{\sigma_z}}

%\renewcommand{\bar}[1]{\overline{#1}}

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{\ensuremath{\mathcal{O}}}
\def\L{\ensuremath{\mathcal{L}}}
\def\calL{{\ensuremath{\cal L}}}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{\ensuremath{\mathcal{S}}}
\def\calA{\ensuremath{\mathcal{A}}}
\def\eps{\varepsilon}
\def\epsK{\varepsilon_K}
\def\epsB{\varepsilon_B}
\def\epsp{\varepsilon^\prime_K}
\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em %%These symbols are already in math set
          \lower.35em\hbox{$\sim$}~}}        %%as \gtrsim and \lesssim
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}}
\def\qsq                {\ensuremath{q^2}}
\def\CP                 {\ensuremath{C\!P}}
%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}}

\def\epstag  {\ensuremath{\epsilon_{\rm tag}}}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}}

% Common combinations
\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}}
\def\sy    {\ensuremath{\sigma_y}}
\def\sz    {\ensuremath{\sigma_z}}

\def\pbcm {\ensuremath{p^*_{B^0}}}
%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}} % dbm

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}}
\newcommand{\Betaprks}{\ensuremath{\bz\ra\etapr\KS}}
\newcommand{\Betaprkz}{\ensuremath{\bz\ra\etapr K^0}}
\newcommand{\etaprepp}{\ensuremath{\etapr\ra\eta\pipi}}
\newcommand{\etaprrg}{\ensuremath{\etapr\ra\rho^0\gamma}}

\newcommand{\inverse}{\ensuremath{^{-1}}}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}}
\newcommand{\chisq}{\ensuremath{\chi^2}}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}}

\newcommand{\dstr}{\ensuremath{D^{*}}}
\newcommand{\dstrstr}{\ensuremath{D^{**}}}
\newcommand{\dsp}{\ensuremath{D^{*+}}}
\newcommand{\dsm}{\ensuremath{D^{*-}}}
\newcommand{\dsz}{\ensuremath{D^{*0}}}

\newcommand{\lum} {\ensuremath{\mathcal{L}}}

\def\rhobar {\ensuremath{\overline \rho}}
\def\etabar {\ensuremath{\overline \eta}}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}},
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|,
|\varepsilon_K|, \Delta m_{B_d}}}

\def\sa{${\sin\! 2 \alpha  }$}
\def\sb{${\sin\! 2 \beta   }$}
\def\sg{${\sin\! 2 \gamma  }$}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }}
\def\stwob{\ensuremath{\sin\! 2 \beta   }}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }}
\def\mistag{\ensuremath{w}}
\def\dilution{\ensuremath{\cal D}}
\def\deltaz{\ensuremath{{\rm \Delta}z}}
\def\deltat{\ensuremath{{\rm \Delta}t}}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}}

\newcommand{\fd}{f_D}
\newcommand{\fds}{f_{D_s}}
\newcommand{\fsubb}{f_B}
\newcommand{\fbd}{f_{B_d}}
\newcommand{\fbs}{f_{B_s}}
\newcommand{\bsubb}{B_B}
\newcommand{\bbd}{B_{B_d}}
\newcommand{\bbs}{B_{B_s}}
\newcommand{\rgbb}{\hat{B}_B}
\newcommand{\rgbbd}{\hat{B}_{B_d}}
\newcommand{\rgbbs}{\hat{B}_{B_s}}
\newcommand{\rgbk}{\hat{B}_K}
\newcommand{\lqcd}{\Lambda_{\mathrm{QCD}}}

\providecommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}






% Journal References
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {#1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {#1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {#1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {#1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {#1}}}
\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{#1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{#1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {#1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {#1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {#1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {A{#1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {#1}}}
\newcommand{\jetp}      [1]  {{JETP~{#1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {G{#1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {#1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {#1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {#1}}}
\providecommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {#1}}}
\newcommand{\nim}       [1]  {{Nucl.\ Instr.\ and Methods~{#1}}}
\newcommand{\nima}      [1]  {{Nucl.\ Instr.\ Methods {A{#1}}}}
\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {#1}}}
\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {B{#1}}}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {#1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B Proc.\ Suppl.\ {#1}}}
\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {#1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {#1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {#1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{#1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{#1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{#1}}}
\providecommand{\pl}        [1]  {{Phys.\ Lett.\ {#1}}}      % dbm
\providecommand{\plb}       [1]  {{Phys.\ Lett.\ B~{#1}}}   % dbm
\providecommand{\prep}      [1]  {{Phys.\ Rep.{#1}}}
\providecommand{\prl}       [1]  {{Phys.\ Rev.\ Lett.\ {#1}}} % dbm
\providecommand{\pr}        [1]  {{Phys.\ Rev.\ {#1}}}
\providecommand{\pra}       [1]  {{Phys.\ Rev.\ A~{#1}}}
\providecommand{\prd}       [1]  {{Phys.\ Rev.\ D~{#1}}}
\providecommand{\pre}       [1]  {{Phys.\ Rev.\ E~{#1}}}
\providecommand{\progtp}    [1]  {{Prog.\ Th.\ Phys.\ {#1}}}
\providecommand{\rmp}       [1]  {{Rev.\ Mod.\ Phys.\ {#1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {#1}}}
\newcommand{\sci}       [1]  {{Science~{#1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {#1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {#1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {#1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {#1}}}
\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{#1}}}
\newcommand{\zp}        [1]  {{Z.\ Phys.\ {#1}}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {#1}}}
\newcommand{\cpc}   [1]  {{Comput.\ Phys.\ Commun.\ {#1}}}
\newcommand{\mpl}     [1]  {{Mod.\ Phys.\ Lett.\ {#1}}}
\newcommand{\fp}       [1]   {{Fortschr.\ Phys.\ {#1}}}
\newcommand{\cnpp}  [1]   {{Comm.\ Nucl.\ Part.\ Phys.\ {#1}}}
\newcommand{\rpp}   [1]    {{Rep.\ Prog.\ Phys.\ {#1}}}
\newcommand{\app}  [1]    {{Acta Phys.\ Polon.\ {#1}}}
\newcommand{\fizika}[1]   {{Fizika~{#1}}}
\newcommand{\spd}  [1]    {{Sov.\ Phys.\ Dokl.\ {#1}}}
\newcommand{\baps} [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {#1}}}
\newcommand{\araa} [1]   {{Ann.\ Rev.\ Astr.\ Ap.\ {#1}}}
\providecommand{\apj} [1]     {{Astro.\ Phys.\ J.\ {#1}}}
\newcommand{\annp}  [1]  {{Ann.\ Phys.\ {#1}}}
\newcommand{\ppnp}  [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {#1}}}
\newcommand{\prsl}  [1]    {{Proc.\ Roy.\ Soc.\ Lond.\ {#1}}}
\newcommand{\apas}  [1]  {{Acta Phys.\ Austr.\ Suppl.\ {#1}}}
\newcommand{\anp}  [1]  {{Adv.\ Nucl.\ Phys.\ {#1}}}
\newcommand{\pan}  [1]  {{Phys.\ Atom.\ Nuclei~{#1}}}
\newcommand{\cmp} [1]  {{Commun.\ Math.\ Phys.\ {#1}}}
\newcommand{\npaps} [1]  {{Nucl.\ Phys.\ A (Proc.\ Suppl.)~{#1}}}

%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}}
\def\bbsim      {\mbox{\tt BBsim}}
\def\beast      {\mbox{\tt Beast}}
\def\beget      {\mbox{\tt Beget}}
\def\Bta        {\mbox{\tt Beta}}
\def\betakfit   {\mbox{\tt BetaKfit}}
\def\cornelius  {\mbox{\tt Cornelius}}
\def\evtgen     {\mbox{\tt EvtGen}}
\def\euclid     {\mbox{\tt Euclid}}
\def\fitver     {\mbox{\tt FitVer}}
\def\fluka          {\mbox{\tt Fluka}}
\def\fortran    {\mbox{\tt Fortran}}
\def\gcalor     {\mbox{\tt GCalor}}
\def\geant      {\mbox{\tt Geant321}}
\def\gheisha    {\mbox{\tt Gheisha}}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}}
\def\minuit     {\mbox{\tt Minuit}}
\def\objegs     {\mbox{\tt Objegs}}
\def\turtle     {\mbox{\tt Decay~Turtle}}
\def\hemicosm   {\mbox{\tt HemiCosm}}
\def\stdhep     {\mbox{\tt StdHep}}
\def\hepevt     {\mbox{\tt{/HepEvt/}}}
\def\squaw      {\mbox{\tt Squaw}}
\def\trackerr   {\mbox{\tt TrackErr}}


==> floatplacement2.tex <==
% floatplacement.tex - Adjust LaTeX ``float'' parameters to afford
%	greater page utilization and minimize float pages at end
%
% Floats are tables and figures which ``float'' around the text page, placed
% where LaTeX things best.  One may select the following ``location'' hints
% for LaTeX: [!htbp], where !=try very hard; h=right Here; t=Top of page; 
% b=Bottom of page; p=place on special Page of floats.
%
% Note that if one uses a location hint of, say, [!htb], then the ``!'' will
% override all placement parameters except for floatpagefraction and 
% dblfloatpagefraction.  Thus, do NOT use the ! except when really necessary.
%
%
%\makeatletter			% ???

% float page layouts
\setcounter{topnumber}{3}	% Max number of top floats per page
\setcounter{dbltopnumber}{3}	%   same for double column pages
\def\topfraction{1.0}		% Max frac of page utilized by top floats
\def\dbltopfraction{1.0}	%   same for double column pages

\setcounter{bottomnumber}{3}	% Max number of bottom floats per page
\def\bottomfraction{1.0}	% Max frac of page utilized by bottom floats
\def\dblbottomfraction{1.0}	%   same for double column pages

\setcounter{totalnumber}{5}	% Max floats per page
\def\textfraction{0.0}		% Min frac of page that must be occupied by text
\def\floatpagefraction{.80}	% Min frac of a float page that must be full
\def\dblfloatpagefraction{.8}	%   same for double column pages


% float positioning
\def\floatsep{1.5cm}		% Space separating top/bottom floats from each other
\def\doublefloatsep{1.5cm}	%   same for double column floats
\def\textfloatsep{0.5cm}	% Space separating top or bottom floats from text
\def\doubletextfloatsep{0.5cm}	%   same for double column floats
\def\intextsep{0.5cm}		% Space separating ``here'' floats from text


% ??? Mysterious stuff in original floatplacement.tex ???
%\@textmin = \textfraction\textheight	%
%\def\fps@figure{tbp}		%
%\def\fps@table{tbp}		%
%\makeatother			%





